VIPeR: Provably Efficient Algorithm for Offline RL with Neural Function Approximation

We propose a novel algorithm for offline reinforcement learning called Value Iteration with Perturbed Rewards (VIPeR), which amalgamates the pessimism principle with random perturbations of the value function. Most current offline RL algorithms explicitly construct statistical confidence regions to obtain pessimism via lower confidence bounds (LCB), which cannot easily scale to complex problems where a neural network is used to estimate the value functions. Instead, VIPeR implicitly obtains pessimism by simply perturbing the offline data multiple times with carefully-designed i.i.d. Gaussian noises to learn an ensemble of estimated state-action {value functions} and acting greedily with respect to the minimum of the ensemble. The estimated state-action values are obtained by fitting a parametric model (e.g., neural networks) to the perturbed datasets using gradient descent. As a result, VIPeR only needs $\mathcal{O}(1)$ time complexity for action selection, while LCB-based algorithms require at least $\Omega(K^2)$, where $K$ is the total number of trajectories in the offline data. We also propose a novel data-splitting technique that helps remove a factor involving the log of the covering number in our bound. We prove that VIPeR yields a provable uncertainty quantifier with overparameterized neural networks and enjoys a bound on sub-optimality of $\tilde{\mathcal{O}}( { \kappa H^{5/2} \tilde{d} }/{\sqrt{K}})$, where $\tilde{d}$ is the effective dimension, $H$ is the horizon length and $\kappa$ measures the distributional shift. We corroborate the statistical and computational efficiency of VIPeR with an empirical evaluation on a wide set of synthetic and real-world datasets. To the best of our knowledge, VIPeR is the first algorithm for offline RL that is provably efficient for general Markov decision processes (MDPs) with neural network function approximation.

==> iclr2023/body/analysis.tex <==
\section{Analysis}

\url{https://math.stackexchange.com/questions/473229/expected-value-of-maximum-and-minimum-of-n-normal-random-variables} 

\begin{hint}
\begin{itemize}
    \item Work with the linear case first 
    \item Utilize the order statistics 
    \item Generalize to NTK? 
\end{itemize}
\end{hint}

We make assumptions on the function class $\mathcal{F}$. 


\begin{assumption}[Completeness]
For any $V: \mathcal{S} \rightarrow [0,H]$ and any $h \in [H]$, $r_h + P_h V \in \mathcal{F}$. 
\end{assumption}

\begin{assumption}[Bounded covering number]
For any $\epsilon > 0$, the covering number $\mathcal{N}(\mathcal{F}, \epsilon)$ is bounded. 
\end{assumption}

% \begin{assumption}[Bounded Eluder dimension]
% For any $V: \mathcal{S} \rightarrow [0,H]$ and any $\mathcal{Z} \in (\mathcal{S} \times \mathcal{A})^{\mathbb{N}}$. Let 
% \begin{align*}
%     \mathcal{F}' := \{f \in \mathcal{F}: \|f - f_V \|_{\mathcal{Z}}^2 + \lambda R(f - f_V) \leq \beta\} 
% \end{align*}
% We assume that $\mathcal{F}'$ has a bounded Eluder dimension. 
% \end{assumption}

Let $\hat{f} := \argmin_{f \in \mathcal{F}} L(f|\mathcal{D})^2 + \lambda R(f)$ be the regularized least-squares solution and $\tilde{f}_{\sigma} := \argmin_{f \in \mathcal{F}} L(f|\tilde{\mathcal{D}}_{\sigma})^2 + \lambda \tilde{R}_{\sigma}(f)$ be the perturbed regularized least-squares solution. For any $v \in (0,1)$, define the anti-concentration width function $g_{\sigma}(\cdot): \mathcal{X} \rightarrow \mathbb{R}$ as 
\begin{align*}
    g_{\sigma}(x) := \sup \{g \in \mathbb{R}: \mathbb{P}\left( \tilde{f}_{\sigma}(x) \leq \hat{f}(x) - g \right) \geq v\}
\end{align*}
Intuitively, $g_{\sigma}(x)$ is the largest gap that $\tilde{f}_{\sigma}(x)$ is smaller than $\hat{f}(x)$ with probability at least $v$. 

\begin{assumption}[Anti-concentration]
Let $\mathcal{F}_{\mathcal{D}, \beta} := \{f \in \mathcal{F}: \|f - \hat{f}\|_{\mathcal{D}}^2 + \lambda R(f - \hat{f}) \leq \beta \}$ be the class of functions that is centered around the regularized least-squares solution $\hat{f}$ within the radius of $
\beta$. We assume that there exists $\sigma > 0$ such that
\begin{align*}
    g_{\sigma'}(x) \geq w_{\mathcal{F}_{\mathcal{D}, \beta}}(x),
\end{align*}
for any $\sigma' \geq \sigma$. 
\label{theorem: anti-cocnetration}
\end{assumption}
The assumption says that the anti-concentration width is as large as the function width. 

\begin{lemma}[Confidence sets around the perturbed regularized least-squares function]
hi
\end{lemma}

We define the model evaluation error at any $(s,a,h) \in \mathcal{S} \times \mathcal{A} \times [H]$ as 
\begin{align}
    \iota_h(s,a) = (T_h \hat{V}_{h+1} - \hat{Q}_h)(s,a). 
    \label{equation: model evaluation error}
\end{align}


We start with the sub-optimality decomposition lemma. 

\begin{lemma}[Sub-optimality decomposition {\citep[Lemma~3.1]{jin2021pessimism}}] 
\begin{align*}
    \subopt(\hat{\pi}; s_1) &= - \sum_{h=1}^H \mathbb{E}_{\hat{\pi}} \left[ \iota_h(s_h, a_h) \right] +  \sum_{h=1}^H \mathbb{E}_{\pi^*} \left[ \iota_h(s_h, a_h) \right] + \sum_{h=1}^H \mathbb{E}_{\pi^*} \left[ \langle \hat{Q}_h(s_h, \cdot), \pi^*_h(\cdot | s_h) - \hat{\pi}_h(\cdot | s_h)
    \rangle_{\mathcal{A}}  \right].
\end{align*}
\end{lemma}

Thus it suffices to prove the following theorem. 
\begin{theorem}[Informal]
With high probability, 
\begin{align*}
   0 \leq \iota_h(s,a) \leq w_{\mathcal{F}}(s,a), \forall (s,a,h). 
\end{align*}
\end{theorem}
\begin{proof}
Let $g_{h, \sigma}$ be a function such that $\tilde{f}^m_h(s,a) \leq \hat{f}_h(s,a) - g_{h, \sigma}(s,a)$ with probability at least $v$ for a fixed $(s,a,h,m)$. As $\{\tilde{f}^m_h\}_{m \in [M]}$ are independent, the probability that there is at least one $m \in [M]$ such that $\tilde{f}^m_h(s,a) \leq \hat{f}_h(s,a) - g_{h, \sigma}(s,a)$ is at least $1 - (1 - v)^M$. By the union bound, with probability at least $1 - HSA (1 - v)^{M}$, for any $(s,a,h) \in \mathcal{S} \times \mathcal{A} \times [H]$, 
\begin{align*}
   \min_{m \in [M]} \tilde{f}^m_h(s,a) \leq \hat{f}_h(s,a) - g_{h, \sigma}(s,a). 
\end{align*}
We set $HSA (1 - v)^M = \delta$, \thanh{the annoying part is that the union over the state and action spaces.} i.e. $M = \log \frac{HSA}{\delta} / \log \frac{1}{1-v}$. Thus, with probability at least $1 - \delta$, for any $(s,a,h)$,  
\begin{align*}
    \tilde{f}_h(s,a) &= \min_{m \in [M]} \tilde{f}^m_h(s,a) \\
    &\leq  \hat{f}_h(s,a) - g_{h, \sigma_h}(s,a) \\ 
    &\leq \hat{f}_h(s,a) - w_{\mathcal{F}_{\mathcal{D}_h, \beta}}(s,a)
\end{align*}
\end{proof}

The idea is that $T_h \hat{V}_{h+1} \approx \langle g(\cdot; w^{(0)}), \bar{w}_h - w^{(0)} \rangle$. Recall that 
\begin{align*}
    \tilde{w}_h &:= \argmin_{w \in \mathbb{R}^{2md}} \sum_{k=1}^K \left( f(s^k_h, a^k_h; b, w) - (r^k_h + \hat{V}_{h+1}(s^k_{h+1}) + \epsilon^{k,i}_h ) \right)^2 + \lambda \| w + \xi^i_h \|_2^2, \\
    \tilde{w}_h^{lin} &:= \argmin_{w \in \mathbb{R}^{2md}} \sum_{k=1}^K \left( \langle g(s^k_h, a^k_h; w^0), w \rangle  - (r^k_h + \hat{V}_{h+1}(s^k_{h+1}) + \epsilon^{k,i}_h ) \right)^2 + \lambda \| w + \xi^i_h \|_2^2
\end{align*}

We want to bound 
\begin{align*}
    \| \tilde{w}_h - \bar{w}_h \|_2 = 
\end{align*}

==> iclr2023/body/linear_case.tex <==
\subsection{The Linear Setting}
\begin{lemma}
Let $\hat{w}_h := \Lambda^{-1}_h \sum_{k=1}^K \phi(s^k_h, a^k_h) \cdot (r^k_h + \tilde{V}_{h+1}(s^k_{h+1}))$ be the non-perturbed regularized least-squares solution at stage $h$. At Line \ref{RAVI-Lin: perturbed ERM} of Algorithm \ref{algorithm: PERVI - Linear MDP}, conditioned on all the randomness except $\{\xi^{k,i}_h\}$ and $\{\zeta^i_h \}$, 
\begin{align*}
    \tilde{w}^i_h - \hat{w}_h \sim \mathcal{N}(0, \sigma^2_h \Lambda_h^{-1}). 
\end{align*}
% \thanh{This makes it become an implicit Thompson sampling. See the Neural Thompson Sampling paper.}
\label{lemma: perturbed weights are Gaussian in linear MDP}
\end{lemma}

\begin{proof}
Let $\bar{w} := w + \zeta^i_h$. Let $f(w) = \sum_{k=1}^K \left(\langle \phi(s^k_h, a^k_h), w \rangle - (r^k_h + \tilde{V}_{h+1}(s^k_{h+1}) + \xi^{k,i}_h ) \right)^2 + \lambda \| w + \zeta^i_h \|_2^2$ and $g(\bar{w}) = \sum_{k=1}^K \left(\langle \phi(s^k_h, a^k_h), \bar{w} \rangle - {y}^k_h \right)^2 + \lambda \| \bar{w}  \|_2^2$, where $y^k_h = r^k_h + \tilde{V}_{h+1}(s^k_{h+1}) + \xi^{k,i}_h + \langle \phi(s^k_h, a^k_h), \zeta^i_h \rangle$. We have $f(w) = g(\bar{w})$ and $\argmax_{w} f(w) = \argmax_{\bar{w}} g(\bar{w}) - \zeta^i_h$ as both $f$ and $g$ are convex. Using the regularized least-squares solution,  
\begin{align*}
     \argmax_{\bar{w}} g(\bar{w}) &= \Lambda_h^{-1} \sum_{k=1}^K \phi(s^k_h, a^k_h) y^k_h \\ 
     &= \Lambda_h^{-1} \left[ \sum_{k=1}^K \phi(s^k_h, a^k_h) (r^k_h + \tilde{V}_{h+1}(s^k_{h+1}) + \xi^{k,i}_h ) + \sum_{k=1}^K \phi(s^k_h, a^k_h) \langle \phi(s^k_h, a^k_h), \zeta^i_h \rangle \right] \\
     &= \Lambda_h^{-1} \left[ \sum_{k=1}^K \phi(s^k_h, a^k_h) (r^k_h + \tilde{V}_{h+1}(s^k_{h+1}) + \xi^{k,i}_h ) + \sum_{k=1}^K \phi(s^k_h, a^k_h) \phi(s^k_h, a^k_h)^T \zeta^i_h  \right] \\ 
     &= \Lambda_h^{-1} \left[ \sum_{k=1}^K \phi(s^k_h, a^k_h) (r^k_h + \tilde{V}_{h+1}(s^k_{h+1}) + \xi^{k,i}_h ) + (\Lambda_h - \lambda I) \zeta^i_h  \right]. 
\end{align*}
Thus, we have
\begin{align*}
    \tilde{w}^i_h &= \argmax_{w} f(w) = \argmax_{\bar{w}} g(\bar{w}) - \zeta^i_h \\
    &=  \Lambda_h^{-1} \left[ \sum_{k=1}^K \phi(s^k_h, a^k_h) (r^k_h + \tilde{V}_{h+1}(s^k_{h+1}) + \xi^{k,i}_h ) + (\Lambda_h - \lambda I) \zeta^i_h  \right] - \zeta^i_h \\
    &= \Lambda_h^{-1} \left[ \sum_{k=1}^K \phi(s^k_h, a^k_h) (r^k_h + \tilde{V}_{h+1}(s^k_{h+1}) + \xi^{k,i}_h )  - \lambda  \zeta^i_h  \right] \\
    &= \hat{w}_h + \Lambda^{-1}_h \left[ \sum_{k=1}^K \phi(s^k_h, a^k_h) \xi^{k,i}_h - \lambda \zeta^i_h \right]
\end{align*}
By direct computation, it is easy to see that 
\begin{align*}
    \tilde{w}^i_h - \hat{w}_h =  \Lambda^{-1}_h \left[ \sum_{k=1}^K \phi(s^k_h, a^k_h) \xi^{k,i}_h - \lambda \zeta^i_h \right] \sim \mathcal{N}(0, \sigma_h^2 \Lambda_h^{-1}). 
\end{align*}

\end{proof}



% Now we prove that with high probability, 
% \begin{align*}
%     \langle \phi(s,a), \hat{w}_h \rangle - \sigma_h \| \phi(s,a) \|_{\Lambda_h^{-1}} \leq (r_h + P_h \tilde{V}_{h+1})(s,a). 
% \end{align*}

% \begin{defn}[Good events]
% For any $\delta > 0$, we define the following events 
% \begin{align*}
%     \mathcal{E}_h(\delta) &:= \left\{ \max_{k \in [K], i \in [M]} |\xi^{k, i}_h| \leq \sqrt{\gamma(\delta)} \land \max_{i \in [M]} \|\zeta^i_h \|_2 \leq \sqrt{\gamma(\delta)} \right\}, \\ 
%     \mathcal{E}(\delta) &:= \bigcap_{h \in [H]} \mathcal{E}_h(\delta),
% \end{align*}
% where $\gamma(\delta)$ is a constant to be specified later. 
% \end{defn}


Let us define the following event
\begin{align*}
    \mathcal{E}(\delta) := \left\{ |\xi^{k,i}_h| \leq c_1 \sigma_h \sqrt{\log (KHM / \delta)} \land \| \zeta^i_h \|_2 \leq c_2 \sigma_h \sqrt{d \log (d KHM / \delta)}: \forall (k,h,i) \in [K] \times [H] \times [M]  \right\},
\end{align*}
for some absolute constant $c_1, c_2 > 0$. 
\begin{lemma}
There exist absolute constants $c_1, c_2 > 0$ such that for any $\delta > 0$, event $\mathcal{E}(\delta)$ holds with probability at least $1 - \delta$. 
\label{Lemma: good events where the noises are bounded}

% with probability at least $1 - \delta$, it hold simultaneously for any $(k,h,i) \in [K] \times [H] \times [M]$,
% \begin{align*}
%     |\xi^{k,i}_h| \leq c_1 \sigma_h \sqrt{\log (KHM / \delta)} \text{ and } \| \zeta^i_h \|_2 \leq c_2 \sigma_h \sqrt{d \log (d KHM / \delta)}. 
% \end{align*}
% \begin{align*}
%     \mathbb{P} \left( \mathcal{E}(\delta)\right) \geq 1 - \delta. 
% \end{align*}
\end{lemma}

\begin{proof}
Use the concentration of multivariate Gaussians from Lemma \ref{lemma: Concentration of multivariate Gaussian}. 
\end{proof}


\begin{lemma}
If $\sigma_h \geq (1 + H) \sqrt{d} + c_3 d H \sqrt{\log (2 d KH /\delta)}$ for any $h$, with high probability $1 - \delta$, it holds simultaneously for all $(s,a,h)$, 
\begin{align*}
   | (r_h + P_h \tilde{V}_{h+1})(s,a) -  \langle \phi(s,a), \hat{\theta}_h \rangle| \leq \sigma_h \| \phi(s,a) \|_{\Lambda_h^{-1}}.  
\end{align*}
\label{lemma: erm within the Bellman target at perturbed}
\end{lemma}

\begin{proof}
As for the linear MDP, by \citep[Lemma~B.1]{jin2021pessimism}, there exists an unknown $\bar{\theta}$ such that 
\begin{align*}
    (r_h + P_h \tilde{V}_{h+1})(s,a) &= \langle \phi(s,a), \bar{\theta}_h \rangle, \forall (s,a), \\
    \| \bar{\theta}_h \| &\leq (1 + H) \sqrt{d}.
\end{align*}
In addition, we have 
\begin{align*}
    \| \hat{\theta}_h \|_2 \leq H \sqrt{Kd /\lambda}. 
\end{align*}

Thus, we have 
\begin{align*}
     &(r_h + P_h \tilde{V}_{h+1})(s,a) - \langle \phi(s,a), \hat{\theta}_h \rangle = \phi(s,a)^T \bar{\theta}_h - \phi(s,a)^T \Lambda^{-1}_h \sum_{k=1}^K \phi(s^k_h, a^k_h) \cdot (r^k_h + \tilde{V}_{h+1}(s^k_{h+1})) \\ 
     &= \underbrace{\phi(s,a)^T \bar{\theta}_h - \phi(s,a)^T \Lambda^{-1}_h \sum_{k=1}^K \phi(s^k_h, a^k_h) \cdot (r_h + P_h \tilde{V}_{h+1})(s^k_h, a^k_h)}_{I_1} \\ 
     &+ \underbrace{\phi(s,a)^T \Lambda^{-1}_h \sum_{k=1}^K \phi(s^k_h, a^k_h) \left[ (r_h + P_h \tilde{V}_{h+1})(s^k_h, a^k_h) - r^k_h - \tilde{V}_{h+1}(s^k_{h+1}) \right]}_{I_2}. 
    %  &= \phi(s,a)^T \bar{w}_h - \phi(s,a)^T \Lambda^{-1}_h \sum_{k=1}^K \phi(s^k_h, a^k_h) \phi(s^k_h, a^k_h)^T \bar{w}_h \\
    %   &+ \phi(s,a)^T \Lambda^{-1}_h \sum_{k=1}^K \phi(s^k_h, a^k_h) \left[ (r_h + P_h \tilde{V}_{h+1})(s^k_h, a^k_h) - r^k_h - \tilde{V}_{h+1}(s^k_{h+1}) \right]
\end{align*}
For term $I_1$, 
\begin{align*}
    I_1 &=  \phi(s,a)^T \bar{\theta}_h - \phi(s,a)^T \Lambda^{-1}_h \sum_{k=1}^K \phi(s^k_h, a^k_h) \phi(s^k_h, a^k_h)^T \bar{\theta}_h \\ 
    &=  \phi(s,a)^T \Lambda_h^{-1} \Lambda_h \bar{\theta}_h - \phi(s,a)^T \Lambda^{-1}_h \sum_{k=1}^K \phi(s^k_h, a^k_h) \phi(s^k_h, a^k_h)^T \bar{\theta}_h \\ 
    &= \lambda \phi(s,a)^T \Lambda_h^{-1}  \bar{\theta}_h \leq \lambda \| \bar{\theta}_h \|_{\Lambda_h^{-1}} \| \phi(s,a) \|_{\Lambda_h^{-1}} \leq  (H + 1) \sqrt{d \lambda} \cdot  \| \phi(s,a) \|_{\Lambda_h^{-1}}. 
\end{align*}
For term $I_2$, by \citep{jin2021pessimism}, with probability at least $1 - \delta$, 
\begin{align*}
    I_2 &\leq  \left\| \sum_{k=1}^K \phi(s^k_h, a^k_h) \left[ (r_h + P_h \tilde{V}_{h+1})(s^k_h, a^k_h) - r^k_h - \tilde{V}_{h+1}(s^k_{h+1}) \right] \right\|_{\Lambda_h^{-1}} \cdot \| \phi(s,a) \|_{\Lambda_h^{-1}} \\ 
    &\leq c_3 d H \sqrt{\log (2 d KH /\delta)} \cdot \| \phi(s,a) \|_{\Lambda_h^{-1}}
\end{align*}

\end{proof}


\begin{lemma}
If we set $M = \log \frac{HSA}{\delta} / \log \frac{1}{1 - \Phi(-1)}$, with probability at least $1 - \delta$, it holds simultaneously for all $(s,a,h)$ that 
\begin{align*}
    \tilde{Q}_h(s,a) \leq \min_{i \in [M]} \langle \phi(s,a), \tilde{\theta}^i_h \rangle \leq \langle \phi(s,a), \hat{\theta}_h \rangle - \sigma_h \| \phi(s,a)\|_{\Lambda_h^{-1}}. 
\end{align*}
\label{lemma: anti-concentration for linear MDP}
\end{lemma}

\begin{proof}
Using the anti-concentration of Gaussian distribution, for any $(s,a) \in \mathcal{S} \times \mathcal{A}$, 
\begin{align*}
    \mathbb{P} \left( \langle \phi(s,a), \tilde{w}^i_h \rangle \leq \langle \phi(s,a), \hat{w}_h \rangle - \sigma_h \| \phi(s,a) \|_{\Lambda_h^{-1}} \right) = \Phi(-1). 
\end{align*}
\end{proof}

From Lemma \ref{lemma: erm within the Bellman target at perturbed}-\ref{lemma: anti-concentration for linear MDP}, with probability at least $1 - 2 \delta$, it holds simultaneously for all $(s,a,h)$ that
\begin{align*}
    \iota_h(s,a) = (r_h + P_h \tilde{V}_{h+1} - \tilde{Q}_h)(s,a) \geq 0.
\end{align*}


\begin{lemma}
With probability at least $1 - 2 \delta$, for any $(s,a,h)$,
\begin{align*}
    0 \leq \iota_h(s,a) \leq (1 + \sqrt{2 \log (1/\delta)}) \sigma_h \cdot \| \phi(s,a)\|_{\Lambda_h^{-1}}. 
\end{align*}
\end{lemma}

\begin{proof}
Let $E_1$ be the event that $\tau_h(s,a) \geq 0, \forall (s,a,h)$. Under event $E_1$, 
\begin{align*}
    \tilde{Q}_h(s,a):=  \min\{ \min_{i \in [M]} \langle \phi(s,a),  \tilde{\theta}_h^i \rangle, H - h +1 \}^+ \leq (r_h + P_h \tilde{V}_{h+1})(s,a) \leq H - h + 1.
\end{align*}
Thus, $\tilde{Q}_h(s,a) = \max\{ \min_{i \in [M]} \langle \phi(s,a),  \tilde{\theta}_h^i \rangle, 0 \}$, and
\begin{align*}
    \iota_h(s,a) &\leq (r_h + P_h \tilde{V}_{h+1} - \hat{Q}_h)(s,a) +  \langle \phi(s,a),  \hat{\theta}_h \rangle - \min_{i \in [M]} \langle \phi(s,a),  \tilde{\theta}_h^i \rangle \\ 
    &\leq \sigma_h \| \phi(s,a)\|_{\Lambda^{-1}_h} + \langle \phi(s,a),  \hat{\theta}_h \rangle - \min_{i \in [M]} \langle \phi(s,a),  \tilde{\theta}_h^i \rangle  \\ 
    &= \sigma_h \| \phi(s,a)\|_{\Lambda^{-1}_h} + \sqrt{2 \log (1 / \delta)}  \sigma_h \| \phi(s,a)\|_{\Lambda^{-1}_h}, 
\end{align*}
where the last inequality is the concentration for a Gaussian variable $\langle \phi(s,a), \hat{\theta}_h - \tilde{\theta}^i_h \rangle$ (Lemma \ref{lemma: perturbed weights are Gaussian in linear MDP}). 
\end{proof}


==> iclr2023/body/notation.tex <==
\section{Notations}
We provide key parameters that we use consistently throughout our proofs. 
\begin{table}[h!]
    \centering
    \begin{tabular}{c|c}
        Notation & Expression \\ 
        \hline
        $\gamma_1(\delta)$ & $c_1 \sigma_h \sqrt{\log (KHM / \delta)}$  \\
        $\gamma_2(\delta)$ & $ c_2 \sigma_h \sqrt{d \log (d KHM / \delta)}$ \\ 
        $\nu$ & $C_g R^{1/3} m^{-1/6} \sqrt{ \log m}$ \\ 
        $B_1$ &  $ \sqrt{K} \nu \sqrt{ (1 + \lambda \eta) ( 2KH^2 + 4 C_g R^{4/3} m^{-1/6} \sqrt{ \log m})}$ \\ 
        $B_2$ &  $K C_g R^{4/3} m^{-1/6} \sqrt{\log m}$ \\ 
        $B_3$ &  $2K \lambda^{-1} H^2 (1 - \eta \lambda)^J$ \\ 
        $\tilde{B}_1$ & $\sqrt{K} \nu \sqrt{ (1 + \lambda \eta) ( \frac{K}{2}(H + \psi + \gamma_{h,1}(\delta) )^2 + \frac{\lambda}{2} \gamma_{h,2}^2(\delta) + 4 C_g R^{4/3} m^{-1/6} \sqrt{ \log m})} $ \\ 
        $\tilde{B}_2$ &  $K C_g R^{4/3} m^{-1/6} \sqrt{\log m}$ \\ 
        $\tilde{B}_3$ & $(1 - \eta \lambda)^J \left( K(H + \psi + \gamma_{h,1}(\delta) )^2 + \gamma_{h,2}^2(\delta) \right)$ \\ 
        $\iota_0$ & $B m^{-1/2} (2 \sqrt{d} + \sqrt{2 \log (1 / \delta)}) $  \\ 
        $\iota_1$ & $C_g R^{4/3} m^{-1/6} \sqrt{ \log m} + C_g \left( \frac{\tilde{B}_1 + \tilde{B}_2}{ \lambda + K C_g^2} + \tilde{B}_3 \right)$  \\ 
        $\iota_2$ & $C_g R^{4/3} m^{-1/6} \sqrt{ \log m} + C_g \left( \frac{{B}_1 + {B}_2}{ \lambda + K C_g^2} + {B}_3 \right)$ \\ 
        $\iota$ & $\iota_0 + \iota_1 + 2 \iota_2$ \\ 
        $\beta$ & $  \frac{B K }{\sqrt{m}} (2 \sqrt{d} + \sqrt{2 \log (4 H /\ \delta)}) \lambda^{-1/2} C_g + \lambda^{1/2}  B + c_3 d H \sqrt{\log (8 d KH / \delta)} $
    \end{tabular}
    \caption{Key parameters in our proofs.}
    \label{tab: key parameters in the proofs}
\end{table}

==> iclr2023/packages.tex <==
% \usepackage[a4paper,top=3cm,bottom=2cm,left=2cm,right=2cm,marginparwidth=1.75cm]{geometry}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[colorlinks=true,linkcolor=blue,citecolor=blue]{hyperref}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{natbib}
\usepackage{bm}
\usepackage{subcaption}
\usepackage{bbm}

%% Additional packages
\usepackage{lmodern}
\usepackage[scale=2]{ccicons}
\usepackage{color}
\usepackage[linewidth=1pt]{mdframed}

\usepackage{booktabs}
% \usepackage[ruled,linesnumbered]{algorithm2e}
\usepackage{tcolorbox}


% \usepackage{algorithm}
% \usepackage{algorithmicx}
% \usepackage{algpseudocode}

\usepackage{amsfonts,amsmath,amssymb,amsthm,mathtools}


\usepackage{xcolor,colortbl}
\usepackage{color}
\usepackage{tcolorbox}
\usepackage{adjustbox}
\usepackage{tabularx}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\newcommand{\hookuparrow}{\mathrel{\rotatebox[origin=c]{90}{$\hookrightarrow$}}}
\newcommand{\hookdownarrow}{\mathrel{\rotatebox[origin=c]{-90}{$\hookrightarrow$}}}

% \newcommand{\question}[1]{\textcolor{red}{\emph{[@\textbf{Question}: #1]}}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\subopt}{SubOpt}
\DeclareMathOperator*{\gap}{gap}
\DeclareMathOperator*{\vect}{vec}

\usepackage{accents}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}

\usepackage{amsmath}
\newcounter{myalgctr}
\numberwithin{enumi}{section}
% https://tex.stackexchange.com/questions/43495/defining-a-custom-environment-with-per-section-numbering

\newenvironment{question}
    {\begin{mdframed}[backgroundcolor=blue!10, linecolor=white]
    \refstepcounter{myalgctr}% increment the environment's counter
    \textbf{Question \themyalgctr}.
        % \begin{quote}
        % \begin{center}
        \begin{em}
    }
    {
        \end{em}
        % \end{center}
        % \end{quote}
        \end{mdframed}
    }

\newenvironment{hint}
{
\begin{mdframed}[backgroundcolor=orange!5, linecolor=white] 
% \refstepcounter{myalgctr}
\textbf{Hint}. 
}
{
\end{mdframed}
}

\newenvironment{todo}
{
\begin{mdframed}[backgroundcolor=red!5, linecolor=white] 
\textbf{TODO}. 
}
{
\end{mdframed}
}


\newcommand{\annoterel}[2]{%
  \overset{%
    \substack{\hidewidth\text{#1}\hidewidth\\\downarrow}%
  }{#2}%
}

% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \usepackage{algorithmicx}
% \usepackage[linesnumbered,ruled]{algorithm2e}
% \newcommand\mycommfont[1]{\ttfamily\textcolor{gray}{#1}}
% \SetCommentSty{mycommfont}
% \SetKwInput{KwInput}{Input}                % Set the Input
% \SetKwInput{KwOutput}{Output}              % set the Output
% \SetKwInput{KwInitialization}{Initialization}
% \SetKwInput{KwRequire}{Require}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{prop}{Proposition}
\newtheorem{observation}{Observation}
\newtheorem{corollary}{Corollary}

\theoremstyle{definition}
\newtheorem{defn}{Definition}
\newtheorem{conj}{Conjecture}[section]
\newtheorem{example}{Example}[section]
\newtheorem{assumption}{Assumption}[section]


\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem*{note}{Note}

\usepackage{xcolor}
\usepackage{enumitem}   

\usepackage{afterpage}

\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage}
    
    
\usepackage{algorithm}
\usepackage{algpseudocode}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\usepackage{minitoc}
\allowdisplaybreaks
% \setlength\parindent{0pt}

%COMMENT 
\newcommand{\thanh}[1]{\textcolor{blue}{\emph{[\textbf{Thanh}: #1]}}}
\newcommand{\raman}[1]{\textcolor{red}{\emph{[\textbf{Raman}: #1]}}}
\newcommand{\cmt}[1]{\textcolor{gray}{\emph{[#1]}}}
% \newcommand{\todoinline}[1]{\textcolor{gray}{#1]}}}
\newcommand{\tO}[1]{\tilde{\mathcal{O}}(}



